Discriminate-and-Rectify Encoders: Learning from Image Transformation Sets

The complexity of a learning task is increased by transformations in the input space that preserve class identity. Visual object recognition for example is affected by changes in viewpoint, scale, illumination or planar transformations. While drastically altering the visual appearance, these changes are orthogonal to recognition and should not be reflected in the representation or feature encoding used for learning. We introduce a framework for weakly supervised learning of image embeddings that are robust to transformations and selective to the class distribution, using sets of transforming examples (orbit sets), deep parametrizations and a novel orbit-based loss. The proposed loss combines a discriminative, contrastive part for orbits with a reconstruction error that learns to rectify orbit transformations. The learned embeddings are evaluated in distance metric-based tasks, such as one-shot classification under geometric transformations, as well as face verification and retrieval under more realistic visual variability. Our results suggest that orbit sets, suitably computed or observed, can be used for efficient, weakly-supervised learning of semantically relevant image embeddings.

==> Orbit Metric Learning (arxiv20170202)_00/fig_mpie_faces.tex <==
% \renewcommand{\fl}{.1\linewidth}

%\renewcommand{\trimmedgraphic}[1]{%
%    \includegraphics[trim = {1cm 1cm 1cm 0.5cm}, clip, width=\linewidth]{#1}%
%}

\begin{figure*}[!ht]
    \begin{center}
        \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-1-canonical}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-5-canonical}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-4-canonical}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-3-canonical}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-2-canonical}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-0-canonical}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ex-best-mistake-1-canonical}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-best-mistake-1-canonical}
        \end{subfigure}%

        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-1-target}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-5-target}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-4-target}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-3-target}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-2-target}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-0-target}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ex-best-mistake-1-target}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-best-mistake-1-target}
        \end{subfigure}%

        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-1-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-5-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-4-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-3-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-2-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-correct-0-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-mistake-1-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ks-best-mistake-1-retrieved}
        \end{subfigure}%

        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ex-correct-1-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ex-correct-5-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ex-correct-4-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ex-correct-3-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ex-correct-2-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ex-correct-0-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ex-best-mistake-1-retrieved}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/ex-mistake-2-retrieved}
        \end{subfigure}%

        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/mpie_rec_2}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/mpie_rec_6}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/mpie_rec_5}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/mpie_rec_4}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/mpie_rec_3}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/mpie_rec_1}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/mpie_rec_8}
        \end{subfigure}%
        \begin{subfigure}{\fl}
            \centering
            \trimmedgraphic{figs/orig/mpie_rec_7}
        \end{subfigure}%
    \end{center}
    % \capmar
    \caption{\small Examples of retrieval and rectification on Multi-PIE. Rows correspond to: 1) canonical pose of the seec image, 2) seed image, 3) Top-1 retrieved using the Orbit Joint (OJ) embedding, 4) Top-1 retrieved using the Exemplar (EX) embedding \cite{Dosovitskiy2015} and 5) the reconstructed canonical pose using the decoder of the OJ network.}
    \label{fig:mpie-data}
\end{figure*}

==> Orbit Metric Learning (arxiv20170202)_00/fig_orbits.tex <==
\begin{figure}[t!]
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/4-000}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/4-045}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/4-090}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/4-135}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/4-180}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/4-225}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/4-270}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/4-315}
    \end{subfigure}%

    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/001_01_01_010_09}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/001_01_01_041_09}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/001_01_01_050_09}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/001_01_01_051_09}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/001_01_01_130_09}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/001_01_01_080_09}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/001_01_01_090_09}
    \end{subfigure}%
    \begin{subfigure}{.125\linewidth}
        \centering
        \includegraphics[width=\linewidth]{orbits/001_01_01_120_09}
    \end{subfigure}%
    \capmar
    \caption{\small Examples of transformation orbits obtained through image rotations/data augmentation (row 1: MNIST, digits) and continuity (row 2: MulitPIE, faces).}
    \label{fig:orbex}
\end{figure}


==> Orbit Metric Learning (arxiv20170202)_00/stn_figure.tex <==
% \newcommand{\fl}{\vspace{-0.5cm}}
\newcommand{\fl}{.1\linewidth}

% \newlength{\cl}{0.5cm}
% \def\cl{0.5cm}
% \includegraphics[trim={5cm 5cm 5cm 0},clip]

\newcommand{\trimmedgraphic}[2][]{%
    \includegraphics[trim = 0cm 0cm 0cm 0cm, clip, width=1\linewidth,#1]%
        {#2}%
}


\begin{figure}[!t]
\begin{center}

\captionsetup[subfigure]{labelformat=empty}
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/input-0048.png}
\end{subfigure}%å
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/input-1062.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/input-0088.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/input-0073.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/input-0002.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/input-0087.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/input-1009.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/input-0101.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/input-0100.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/input-0017.png}
\end{subfigure}%
\vspace{-0.1cm}
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/triplet-stn-0048.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/triplet-stn-1062.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/triplet-stn-0088.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/triplet-stn-0073.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/triplet-stn-0002.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/triplet-stn-0087.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/triplet-stn-1009.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/triplet-stn-0101.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/triplet-stn-0100.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/triplet-stn-0017.png}
\end{subfigure}%
\vspace{-0.1cm}
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/orbit-loss-stn-0048.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/orbit-loss-stn-1062.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/orbit-loss-stn-0088.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/orbit-loss-stn-0073.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/orbit-loss-stn-0002.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/orbit-loss-stn-0087.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/orbit-loss-stn-1009.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/orbit-loss-stn-0101.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/orbit-loss-stn-0100.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/orbit-loss-stn-0017.png}
\end{subfigure}%
\vspace{-0.1cm}
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/ks-0048.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/ks-1062.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/ks-0088.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/ks-0073.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/ks-0002.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/ks-0087.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/ks-1009.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/ks-0101.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/ks-0100.png}
\end{subfigure}%
\begin{subfigure}{\fl}
  \centering
 \trimmedgraphic{figs/stn/ks-0017.png}
\end{subfigure}%
%\vspace{-0.1cm}
\end{center}
\capmar \capmar
\caption{\small % We STN to our model and trained with ST (full supervision) and OT (weak supervision). 
Input (row 1) and rectifications for ST-STN (row 2), OT-STN (row 3) and OJ (row 4). STNs produced convincing rectifications when full supervision was available (ST-STN) but learned the identity with weak supervision (OT-STN). The encoder-decoder map trained with the proposed orbit metric loss produces accurate rectifications using only weak supervision.}
\label{fig:stn-rec}
% \vspace{-0.4cm}
\end{figure}

